SegNeRF: 3D Part Segmentation with Neural Radiance Fields

Recent advances in Neural Radiance Fields (NeRF) boast impressive performances for generative tasks such as novel view synthesis and 3D reconstruction. Methods based on neural radiance fields are able to represent the 3D world implicitly by relying exclusively on posed images. Yet, they have seldom been explored in the realm of discriminative tasks such as 3D part segmentation. In this work, we attempt to bridge that gap by proposing SegNeRF: a neural field representation that integrates a semantic field along with the usual radiance field. SegNeRF inherits from previous works the ability to perform novel view synthesis and 3D reconstruction, and enables 3D part segmentation from a few images. Our extensive experiments on PartNet show that SegNeRF is capable of simultaneously predicting geometry, appearance, and semantic information from posed images, even for unseen objects. The predicted semantic fields allow SegNeRF to achieve an average mIoU of $\textbf{30.30%}$ for 2D novel view segmentation, and $\textbf{37.46%}$ for 3D part segmentation, boasting competitive performance against point-based methods by using only a few posed images. Additionally, SegNeRF is able to generate an explicit 3D model from a single image of an object taken in the wild, with its corresponding part segmentation.

==> supplmat/0_dataset.tex <==
\section{Dataset Details}
\label{sec:dataset}
We present the abbreviation for some of the categories reported in the main manuscript in \Table{dataset_abrev}.
\begin{table}[ht]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|lllllll}\Xhline{2\arrayrulewidth}
\textbf{Abbreviation} & \bfseries Bott  & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Micro & \bfseries Stora \\\Xhline{2\arrayrulewidth}
\textbf{Full Name} &bottle & dishwasher & display & earphones & faucet & microwave & storage furniture\\\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\textbf{Category abbreviation.} The complete name for the reported categories in the main manuscript.}
\label{tab:dataset_abrev}
\end{table}

%The results of the remaining categories and the details of training and validation splits are described in the~\SM.
We give additional details on the number of distinct shape instances remaining from each category remaining after matching objects from PartNet with their corresponding objects in ShapeNet in \Table{dataset}. We maintain above 90\% categories such as: chair, clock, display, faucet, storage furniture, table, trash, and vase. On the other hand, these categories are below 90\%: bed, bottle, dishwasher, earphones, knife, and microwave. 
% \subsection{Splits}
\begin{table}[ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccccccccccccc}\Xhline{2\arrayrulewidth}
  &\bfseries Total &\bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase \\\Xhline{2\arrayrulewidth}
\textbf{PartNet} &22508 &    248  & 519      &6400       &579       &201      &954      &247      &708       &384  &212  & 2303 & 8309 & 340 & 1104\\
\textbf{Ours}   &21468&  192   &  435     &  6311     &     552  &  82    &927      &68      &   648    &326 & 120  &2243  & 8179 & 321 &1064   \\\hline
\textbf{Percentage} & 95.3 & 77.4 &  83.8 & 98.6 & 95.3 & 40.7 & 97.8 & 27.5 & 91.5 & 84.9 & 56.6 & 97.3 & 98.4 & 94.4 & 96.4  \\\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\textbf{PartNet subset statistics.} Number of distinct shape instances for the complete PartNet dataset and the subset utilized in this paper. Additionally, the percentage of the comparison between the complete PartNet dataset and ours.}
\label{tab:dataset}
\end{table}

The categories that are not taken into account for the experiments are: bag, bowl, door, hat, key lamp, laptop, mug, fridge, and scissors.
The total number of instances that are within these categories is 4163 (15\% from the original PartNet dataset).

==> supplmat/1_trainingdet.tex <==
\section{Training Details}
\subsection{SegNeRF Architecture}
% Network $\mathcal{H}$ is composed of 3 fully connected layers with residual connections and width $512$.
% Network $\mathcal{G}$ is composed of 2 fully connected layers with residual connections and width $512$.
We follow the training procedure from~\cite{pixelnerf}, the encoder $\mathcal{E}$ is a ResNet34 backbone and extract a feature pyramid by taking the feature maps before to the first pooling operation and after the first ResNet 3 layers.
Network $\mathcal{H}$ is composed of 3 fully connected layers while network $\mathcal{G}$ is made up of 2 fully connected layers.
All layers use residual connections and have a hidden dimension of $512$.
We use ReLU activations before every fully connected layer.
The positional encoding comprises six exponentially increasing frequencies for each input coordinate. 

We train for 600000 iterations, which took roughly 6 days on 4 V100 NVIDIA GPU.

\subsection{2D Novel-View Part Segmentation}
\mysection{DeepLab v3} 
We train one model per category for 20 epochs (max. one day in 4 V100 NVIDIA GPUs) with a batch size of 100.
Additionally, the model expects input normalized images, \ie mini-batches of 3-channel RGB images of shape (N, 3, H, W), where N is the number of images, H and W are the height, and width of the images. 
The images have to be loaded in to a range of [0, 1] and then normalized using mean = [0.5, 0.5, 0.5] and std = [0.5, 0.5, 0.5].

DeepLab v3 returns an OrderedDict with two Tensors of the same height and width as the input Tensor, but with 21 classes. output['out'] contains the semantic masks, and output['aux'] contains the auxiliary loss values per-pixel.
We remove the last layer of 21 classes and replace it with the number per category.
In inference mode, output['aux'] is not useful. So, output['out'] is shaped (N, C, H, W). C being the classes per category and the desired resolution. 
The resolution was the finest level (3).

We utilize a ResNet-50 backbone, and the model was pre-trained on COCO 2017.
Lastly, we use Adam optimizer, and cosine annealing LR scheduler with $T\_max=10$ were used.

\subsection{Single/Multi-View 3D Part Segmentation}
\mysection{PointNet} and \mysection{PointNet++}
We follow the training procedure from~\cite{pointnet} and \cite{PointNet++}, respectively.
We train only one model for all categories for 251 epochs (2 days in 1 V100 NVIDIA GPU).
The batch size was 45 and 25 for PointNet and PointNet++ models, respectively.
Additionally, each model expects as input normalized point clouds, \ie mini-batches of objects in a range of [0, 1]. 
We utilize Adam optimizer with learning rate $0.001$, betas of $(0.9, 0.999)$ and weight decay of $0.5$.
Both models were initialized with Xavier uniform initialization.
Lastly, we use PointNet++ MSG version.

\mysection{PosPool} We follow the training procedure from~\cite{CloserLook3D}, and train their architecture variant which uses sinusoidal positional embedding, $\text{PosPool}^*$.
\subsection{Single/Multi-View 3D Reconstruction}

\mysection{SoftRas}
We follow the training procedure from~\cite{SoftRas}, we train one model for \textit{chair}, \textit{table}, and all categories.
In the main manuscript, the reported results are with \textit{chair} and \textit{table} models that were trained for 250000 iterations. 
In \SM, we detail results for \textit{all} categories model that was trained for 500000 iterations.
We utilize Adam optimizer with learning rate $0.0001$, betas of $(0.9, 0.999)$.


==> supplmat/2_results.tex <==
% Additional metrics such as accuracy and mean accuracy are reported in the \SM.
\section{Additional Results}
\subsection{2D Novel-View Part Segmentation}

In \Figure{2D_mIoU_lv3_qualitative_sm_table} and \Figure{2D_mIoU_lv3_qualitative_sm_chair}, we show additional result for \textit{table} and \textit{chair} categories. These examples were randomly selected.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{supplmat/imgs/seg_2d_sm_table.pdf}
    \caption{
    \textbf{Additional 2D semantic part segmentation for novel views (\textit{table}) results.} 
     Qualitative results for 2D semantic part segmentation for novel views.
    }
    \label{fig:2D_mIoU_lv3_qualitative_sm_table}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{supplmat/imgs/seg_2d_sm_chair.pdf}
    \caption{
    \textbf{Additional 2D semantic part segmentation for novel views (\textit{chair}) results.} 
     Qualitative results for 2D semantic part segmentation for novel views.
    }
    \label{fig:2D_mIoU_lv3_qualitative_sm_chair}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Single/Multi-View 3D Part Segmentation}



In \Figure{3D_mIoU_lv3_qualitative_sm}, we show additional result for all categories. These examples were randomly selected.

\begin{figure}[ht]{
    \centering
    \includegraphics[width=\linewidth]{supplmat/imgs/AllQual_seg_3D.pdf}}
     \caption{
    \textbf{Additional 3D Semantic Part Segmentation from Multiple Images Results.} 
     Qualitative results for 3D semantic part segmentation from four input source views.
    %  From left to right in each clu: source views, ground truth, \MV, Ours, PosPool\cite{CloserLook3D}.
    }
    \label{fig:3D_mIoU_lv3_qualitative_sm}
\end{figure}



\Table{3D_acc_lv3} and \Table{3D_macc_lv3} report accuracy and mean accuracy for all methods.



\begin{table}[ht]
    \resizebox{\textwidth}{!}{
        
            
            \csvreader[
            tabular=l|c|cccccccccccccc,
            table head=\Xhline{2\arrayrulewidth}\bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase\\\Xhline{2\arrayrulewidth},
            late after line=\ifnumequal{\thecsvrow}{8}{\\\hdashline}{\\},
            table foot=\Xhline{2\arrayrulewidth},
            head to column names,]{results/3D_acc_max_level_3_supp.csv}{}
            {\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \microwave & \storagefurniture & \tables & \trashcan & \vase}
       
    }
    \caption{\textbf{Fine-grained 3D semantic segmentation (3D part-category accuracy\%).} Quantitative results for fine-grained 3D semantic segmentation are presented, with a detailed breakdown by category. Our method outperforms the 2D-supervised methods by significant margins in all categories, and attains comparable results with 3D-supervised methods.}
    \label{tab:3D_acc_lv3}
\end{table}

\begin{table}[ht]
    \resizebox{\textwidth}{!}{
        
            
            \csvreader[
            tabular=l|c|cccccccccccccc,
            table head=\Xhline{2\arrayrulewidth}\bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase\\\Xhline{2\arrayrulewidth},
            late after line=\ifnumequal{\thecsvrow}{8}{\\\hdashline}{\\},
            table foot=\Xhline{2\arrayrulewidth},
            head to column names,]{results/3D_macc_max_level_3_supp.csv}{}
            {\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \microwave & \storagefurniture & \tables & \trashcan & \vase}
       
    }
    \caption{\textbf{Fine-grained 3D semantic segmentation (3D part-category mean accuracy\%).} Quantitative results for fine-grained 3D semantic segmentation are presented, with a detailed breakdown by category. Our method outperforms the 2D-supervised methods by significant margins in all categories, and attains comparable results with 3D-supervised methods.}
    \label{tab:3D_macc_lv3}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Single/Multi-View 3D Reconstruction}

In \Figure{3D_rec_qualitative_sm_table} and \Figure{3D_rec_qualitative_sm_chair}, we show additional result for \textit{table} and \textit{chair} categories. These examples were randomly selected.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{supplmat/imgs/rec_3D_sm_table.pdf}
    \caption{\textbf{Additional 3D Reconstruction from Single Image Results.} Qualitative results for 3D reconstruction are presented for \textit{table}.}
    \label{fig:3D_rec_qualitative_sm_table}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{supplmat/imgs/rec_3D_sm_chair.pdf}
    \caption{\textbf{Additional 3D Reconstruction from Single Image Results.} Qualitative results for 3D reconstruction are presented for \textit{chair}.}
    \label{fig:3D_rec_qualitative_sm_chair}
\end{figure}

\subsection{Semantic Reconstruction}
We combine 3D reconstruction and semantic segmentation by first reconstructing objects into a mesh.
Vertices from the mesh are then colored according to the 3D segmentation predicted by SegNeRF at each of the vertex locations.
The resulting is a semantic reconstruction mesh which can be segmented into each of the object's parts.
Please see the supplementary video for visualizations on semantic reconstructions of chair objects from $4$ source images, which showcases the ability of SegNeRF to perform joint 3D reconstruction and segmentation.
% \Table{3D_rec_ch} and \Table{3D_rec_fs} report chamfer distance and f-score for all methods and categories.

% \begin{table}[ht]
%     \resizebox{\textwidth}{!}{
        
            
%             \csvreader[
%             tabular=l|c|cccccccccccccc,
%             table head=\Xhline{2\arrayrulewidth}\bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase\\\Xhline{2\arrayrulewidth},
%             late after line=\ifnumequal{\thecsvrow}{4}{\\\hdashline}{\\},
%             before line=\ifnumequal{\thecsvrow}{7}{\hdashline}{},
%             table foot=\Xhline{2\arrayrulewidth},
%             head to column names,]{results/3D_rec_supp.csv}{}
%             {\bfseries\Name & \avgchamfer & \bedchamfer & \bottlechamfer &  \chairchamfer & \clockchamfer & \dishwasherchamfer & \displaychamfer & \earphonechamfer & \faucetchamfer & \knifechamfer & \microwavechamfer & \storagefurniturechamfer & \tableschamfer & \trashcanchamfer & \vasechamfer}
       
%     }
%     \caption{\textbf{3D reconstruction (Chamfer Distance $\downarrow$).} Quantitative results for 3D reconstruction for all categories are presented.}
%     \label{tab:3D_rec_ch}
% \end{table}

% \begin{table}[ht]
%     \resizebox{\textwidth}{!}{
        
            
%             \csvreader[
%             tabular=l|c|cccccccccccccc,
%             table head=\Xhline{2\arrayrulewidth}\bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase\\\Xhline{2\arrayrulewidth},
%             late after line=\ifnumequal{\thecsvrow}{4}{\\\hdashline}{\\},
%             before line=\ifnumequal{\thecsvrow}{7}{\hdashline}{},
%             table foot=\Xhline{2\arrayrulewidth},
%             head to column names,]{results/3D_rec_supp.csv}{}
%             {\bfseries\Name & \avgf & \bedf & \bottlef &  \chairf & \clockf & \dishwasherf & \displayf & \earphonef & \faucetf & \knifef & \microwavef & \storagefurnituref & \tablesf & \trashcanf & \vasef}
       
%     }
%     \caption{\textbf{3D reconstruction (F-Score $\uparrow$).} Quantitative results for 3D reconstruction for all categories are presented.}
%     \label{tab:3D_rec_fs}
% \end{table}

==> supplmat/4_real.tex <==
\section{Varying Reconstruction Threshold}
\section{Reconstruction With vs. Without Segmentation}
\section{Real-world images}
\section{Non-zero d for 3D}

==> tables/3D_rec.tex <==
% \begin{table}[htb]

%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|c|c|c|c|c|c|c|c}\Xhline{2\arrayrulewidth}
    
%       & \multicolumn{4}{c|}{\textbf{Chairs}} & \multicolumn{4}{c}{\textbf{Tables}}  \\ \hline
%          & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$  & \bfseries Precision $\uparrow$ & \bfseries Recall $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$   & \bfseries Precision $\uparrow$  & \bfseries Recall $\uparrow$ 
%         \csvreader[head to column names]{results/3D_rec.csv}{}
%         {\\\hline \bfseries \Name &  \chairchamfer &  \chairf &  \chairr &  \chairp & \tableschamfer & \tablesf & \tablesr & \tablesp } \\\Xhline{2\arrayrulewidth}
        
%     \end{tabular}
%     }
%     \caption{3D Rec}
%     \label{tab:3D_rec}
% \end{table}
%late after line=\ifnumequal{\thecsvrow}{2}{\\\hdashline}{\\},
% \begin{table}[htb]

%     \centering
%     \resizebox{0.9\textwidth}{!}{
%         \csvreader[tabular=c|c|c|c|c|c|c|c|c,
%         table head=\Xhline{2\arrayrulewidth} & \multicolumn{4}{c|}{\textbf{Chairs}} & \multicolumn{4}{c}{\textbf{Tables}} \\ & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$  & \bfseries Precision $\uparrow$ & \bfseries Recall $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$   & \bfseries Precision $\uparrow$  & \bfseries Recall $\uparrow$\\\Xhline{2\arrayrulewidth},
%         table foot=\Xhline{2\arrayrulewidth},
%         head to column names]{results/3D_rec_test.csv}{}
%         {\bfseries \Name &  \chairchamfer &  \chairf &  \chairr &  \chairp & \tableschamfer & \tablesf & \tablesr & \tablesp }
        
    
%     }
%     \caption{3D Rec}
%     \label{tab:3D_rec}
% \end{table}

\begin{table}[t]

    \centering
    \resizebox{0.47\textwidth}{!}{
        \csvreader[tabular=c|c|c|c|c|c|c|c|c,
        table head=\Xhline{2\arrayrulewidth} & \multicolumn{4}{c|}{\textbf{Chair}} & \multicolumn{4}{c}{\textbf{Table}} \\ & \bfseries CD $\downarrow$ & \bfseries F-Sc $\uparrow$  & \bfseries P $\uparrow$ & \bfseries R $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Sc $\uparrow$   & \bfseries P $\uparrow$  & \bfseries Re $\uparrow$\\\Xhline{2\arrayrulewidth},
        table foot=\Xhline{2\arrayrulewidth},
        head to column names]{results/3D_rec_val.csv}{}
        {\bfseries \Name &  \chairchamfer &  \chairf &  \chairr &  \chairp & \tableschamfer & \tablesf & \tablesr & \tablesp }
    }
     \caption{\textbf{3D Reconstruction from Single Image.} Quantitative results for 3D reconstruction are presented for the \emph{chair} and \emph{table} categories. Metrics set key: \textbf{CD}: Chamfer distance., \textbf{F-Sc}: F-Score, \textbf{P}: Precision, \textbf{R}: Recall.}
    \label{tab:3D_rec}
\end{table}

% \begin{table}[htb]

%     \centering
%     \resizebox{0.9\textwidth}{!}{
%         \csvreader[tabular=c|c|c|c|c|c|c|c|c,
%         table head=\Xhline{2\arrayrulewidth} & \multicolumn{4}{c|}{\textbf{Chairs}} & \multicolumn{4}{c}{\textbf{Tables}} \\ & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$  & \bfseries Precision $\uparrow$ & \bfseries Recall $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$   & \bfseries Precision $\uparrow$  & \bfseries Recall $\uparrow$\\\Xhline{2\arrayrulewidth},
%         table foot=\Xhline{2\arrayrulewidth},
%         head to column names]{results/3D_rec_postprocess.csv}{}
%         {\bfseries \Name &  \chairchamfer &  \chairf &  \chairr &  \chairp & \tableschamfer & \tablesf & \tablesr & \tablesp }
        
    
%     }
%     \caption{3D Rec with postprocessing}
%     \label{tab:3D_rec_postprocess}
% \end{table}



%& \multicolumn{4}{c|}{\textbf{Chairs}} & \multicolumn{4}{c}{\textbf{Tables}}  \\ 
        %  & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$  & \bfseries Precision $\uparrow$ & \bfseries Recall $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$   & \bfseries Precision $\uparrow$  & \bfseries Recall $\uparrow$ \\\Xhline{2\arrayrulewidth}

==> tables/MultiView.tex <==
% \begin{table}[htb]

%     \centering
%     \resizebox{0.9\textwidth}{!}{
%         \csvreader[tabular=c|c|c|c|c|c|c|c|c,
%         table head=\Xhline{2\arrayrulewidth} & \multicolumn{4}{c|}{\textbf{Chairs}} & \multicolumn{4}{c}{\textbf{Tables}} \\ & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$  & \bfseries Precision $\uparrow$ & \bfseries Recall $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Score $\uparrow$   & \bfseries Precision $\uparrow$  & \bfseries Recall $\uparrow$\\\Xhline{2\arrayrulewidth},
%         table foot=\Xhline{2\arrayrulewidth},
%         head to column names]{results/3D_rec_num_test.csv}{}
%         {\bfseries \Name &  \chairchamfer &  \chairf &  \chairr &  \chairp & \tableschamfer & \tablesf & \tablesr & \tablesp }
        
    
%     }
%     \caption{3D Rec}
%     \label{tab:3D_rec_num}
% \end{table}


\begin{table}[t]

    \centering
    \resizebox{0.47\textwidth}{!}{
        \csvreader[tabular=c|c|c|c|c|c|c|c|c,
        table head=\Xhline{2\arrayrulewidth} & \multicolumn{4}{c|}{\textbf{Chairs}} & \multicolumn{4}{c}{\textbf{Tables}} \\ & \bfseries CD $\downarrow$ & \bfseries F-Sc $\uparrow$  & \bfseries P $\uparrow$ & \bfseries R $\uparrow$   & \bfseries CD $\downarrow$ & \bfseries F-Sc $\uparrow$   & \bfseries P $\uparrow$  & \bfseries R $\uparrow$\\\Xhline{2\arrayrulewidth},
        % late after line=\ifnumequal{\thecsvrow}{5}{\\\hdashline}{\\},
        late after line=\ifnumequal{\thecsvrow}{5}{\\\hdashline}{\\},
        before line=\ifnumequal{\thecsvrow}{7}{\hdashline}{},
        % late after line=\ifnumequal{\thecsvrow}{7}{\\\hdashline}{\\},
        table foot=\Xhline{2\arrayrulewidth},
        head to column names]{results/3D_rec_num_val_v2.csv}{}
        {\bfseries \Name &  \chairchamfer &  \chairf &  \chairr &  \chairp & \tableschamfer & \tablesf & \tablesr & \tablesp }
        
    
    }
   \caption{\textbf{3D Reconstruction from Multiple Images.} We present quantitative results for 3D reconstruction, with a varying number of input images (in parenthesis). Using multiple images results in a much higher quality of reconstruction. Metrics set key: \textbf{CD}: Chamfer distance., \textbf{F-Sc}: F-Score, \textbf{P}: Precision, \textbf{R}: Recall.}
    \label{tab:3D_rec_num}
\end{table}



==> tables/others.tex <==
% \begin{table}[htb]
%     \centering
%     \begin{tabular}{||c|c|c|c|c||} \hline
%          Method       & Coarse  & Fine \\ \hline
%          PointNet     & 64.6 & 27.8 \\ \hline
%          PointNet++   & 68 & 39.2                                     \\ \hline
%          SpiderCNN       & 67.4 & 30.0 \\ \hline
%          PointCNN & 69.6 & 43.9  \\ \hline
%          PosPool & - & 50.8  \\ \hline
%          MV (1 image) & - & -  \\ \hline
%          MV (250 images) & 55.23 & -  \\ \hline
%          SegNerf (ours) (1 image) & 57.84 & 33.05  \\ \hline
%          SegNerf (ours) (2 images) & 63.31 & 36.77  \\ \hline

%     \end{tabular}
%     \caption{Caption}
%     \label{tab:3D_Segmentation}
% \end{table}

% \begin{table}[htb]
%     \centering
%     \begin{tabular}{||c|c|c|c|c||} \hline
%           & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c||}{Tables}  \\ \hline
%          Method         & CD    & F-Score & CD  & F-Score \\ \hline
%          SoftRas        &       &         &     &  \\ \hline
%          DVR            & 57.84 & 33.05   &     &  \\ \hline
%          SegNerf (ours) & 57.84 & 33.05   &     &  \\ \hline
%          Unisurf (ours) & 63.31 & 36.77   &     &  \\ \hline

%     \end{tabular}
%     \caption{Caption}
%     \label{tab:3D_Reconstruction}
% \end{table}

% \begin{table}[htb]
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{l|c|ccccccccccccccc}%
%             \bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Lamp & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase
%             \csvreader[head to column names]{results/3D_miou_max_level_1.csv}{}
%             {\\\hline\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \lamp & \microwave & \storagefurniture & \tables & \trashcan & \vase}
%         \end{tabular}
%     }
%     \caption{Coarse 3D mIoU}
%     \label{tab:3D_mIoU_lv1}
% \end{table}

% \begin{table}[htb]
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{l|c|ccccccccccccccc}%
%             \bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Lamp & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase
%             \csvreader[head to column names]{results/step_max_level_3.csv}{}
%             {\\\hline\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \lamp & \microwave & \storagefurniture & \tables & \trashcan & \vase}
%         \end{tabular}
%     }
%     \caption{Fine num val steps}
%     \label{tab:val_steps_lv3}
% \end{table}

% \begin{table}[htb]
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{l|c|ccccccccccccccc}%
%             \bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Lamp & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase
%             \csvreader[head to column names]{results/step_max_level_1.csv}{}
%             {\\\hline\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \lamp & \microwave & \storagefurniture & \tables & \trashcan & \vase}
%         \end{tabular}
%     }
%     \caption{Coarse num val steps}
%     \label{tab:val_steps_lv1}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% REMOVED LAMP
% \begin{table}[htb]
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{l|c|ccccccccccccccc}%
%             \bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase
%             \csvreader[head to column names]{results/step_max_level_3.csv}{}
%             {\\\hline\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \microwave & \storagefurniture & \tables & \trashcan & \vase}
%         \end{tabular}
%     }
%     \caption{Fine num val steps}
%     \label{tab:val_steps_lv3}
% \end{table}

% \begin{table}[htb]
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{l|c|ccccccccccccccc}%
%             \bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife  & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase
%             \csvreader[head to column names]{results/step_max_level_1.csv}{}
%             {\\\hline\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \microwave & \storagefurniture & \tables & \trashcan & \vase}
%         \end{tabular}
%     }
%     \caption{Coarse num val steps}
%     \label{tab:val_steps_lv1}
% \end{table}

% \begin{table}[htb]
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{l|c|ccccccccccccccc}%
%             \bfseries & \bfseries Avg  & \bfseries Bed & \bfseries Bott  & \bfseries Chair & \bfseries Clock & \bfseries Dish & \bfseries Disp & \bfseries Ear & \bfseries Fauc & \bfseries Knife & \bfseries Lamp & \bfseries Micro & \bfseries Stora & \bfseries Table & \bfseries Trash & \bfseries Vase
%             \csvreader[head to column names]{results/step_max_level_1.csv}{}
%             {\\\hline\bfseries\Name & \avg & \bed & \bottle &  \chair & \clock & \dishwasher & \display & \earphone & \faucet & \knife & \lamp & \microwave & \storagefurniture & \tables & \trashcan & \vase}
%         \end{tabular}
%     }
%     \caption{Coarse num val steps}
%     \label{tab:val_steps_lv1}
% \end{table}

